What Does Success Look Like? Catalyzing Meeting Intentionality with AI-Assisted Prospective Reflection

Despite decades of HCI and Meeting Science research, complaints about ineffective meetings are still pervasive. We argue that meeting technologies lack support for prospective reflection, that is, thinking about why a meeting is needed and what might happen. To explore this, we designed a Meeting Purpose Assistant (MPA) technology probe to coach users to articulate their meeting's purpose and challenges, and act accordingly. The MPA used Generative AI to support personalized and actionable prospective reflection across the diversity of meeting contexts. Using a participatory prompting methodology, 18 employees of a global technology company reflected with the MPA on upcoming meetings. Observed impacts were: clarifying meeting purposes, challenges, and success conditions; changing perspectives and flexibility; improving preparation and communication; and proposing changed plans. We also identify perceived social, temporal, and technological barriers to using the MPA. We present system and workflow design considerations for developing AI-assisted reflection support for meetings.

==> _macros.tex <==

%\usepackage[dvipsnames]{xcolor}
\usepackage{xcolor}

\newcommand{\pid}[1]{{\fontfamily{cmss}\selectfont{\footnotesize{{\textcolor{black!50}{#1}}}}}}

\newcommand{\mpa}[1]{{\fontfamily{cmss}\selectfont{\footnotesize{{\color{violet}{#1}}}}}}

 

\newcommand{\iquotempa}[1]{{\small\fontfamily{cmss}\selectfont\textit{\color{violet}{#1}}}}


\newcommand{\iquote}[1]{\textit{\color{blue}{#1}}}

\newenvironment{smallquote}
  {\begin{quote}\normalsize}
  {\end{quote}}

\newtoggle{comments}
\toggletrue{comments}

\iftoggle{comments} {
\newcommand{\lev}[1]{{\color{red}{LT: #1}\normalfont}}
\newcommand{\sean}[1]{{\color{magenta}{SR: #1}\normalfont}}
\newcommand{\ava}[1]{{\color{cyan}{AS: #1}\normalfont}}
\newcommand{\panda}[1]{{\color{green}{PP: #1}\normalfont}}
}{
  \newcommand {\lev}[1]{}
  \newcommand {\sean}[1]{}
  \newcommand {\ava}[1]{}
  \newcommand {\panda}[1]{}
 }


==> zzzsubs.tex <==
Our findings underscored the lack of intentionality in meetings... \lev{TODO} [SEAN IS WORKING ON THIS - putting together a para from  5.2.1, 5.2.3, 5.2.5, 5.2.6, 5.3.1,  5.3.2, 5.3.3, 5.5.1, 5.5.2]

Our findings underscore the pervasive lack of intentionality in meetings, as evidenced by participants' reflections on their broader meeting experiences. Participants highlighted how translating implicit goals into explicit ones helped clarify understanding and consolidate focus, suggesting that many of their regular meetings lacked clear, articulated purposes (\ref{Making Purpose Explicit}). The "Prioritization" section revealed that while prioritizing discussion topics can be beneficial, it often does not lead to specific, operationalized goals, indicating a common issue in their usual meetings where priorities are not clearly defined 1. Additionally, the "Reflecting on Unknown Variables" section showed that participants had varying levels of appetite for anticipating alternative scenarios, reflecting a general lack of preparedness and foresight in their typical meetings 1. The "Therapy and Coaching" section described how the MPA felt like interacting with a therapist or coach, helping reduce anxiety and stress, which implies that their regular meetings often induce anxiety and lack supportive structures 1. Finally, the "Changing Perspectives and Flexibility" section illustrated how considering other attendees' perspectives can lead to better collaboration and flexibility, though it can also make participants less flexible in certain meetings, highlighting the need for more adaptive and empathetic meeting practices 1.

